NeAI: A Pre-convoluted Representation for Plug-and-Play Neural Ambient Illumination

Recent advances in implicit neural representation have demonstrated the ability to recover detailed geometry and material from multi-view images. However, the use of simplified lighting models such as environment maps to represent non-distant illumination, or using a network to fit indirect light modeling without a solid basis, can lead to an undesirable decomposition between lighting and material. To address this, we propose a fully differentiable framework named neural ambient illumination (NeAI) that uses Neural Radiance Fields (NeRF) as a lighting model to handle complex lighting in a physically based way. Together with integral lobe encoding for roughness-adaptive specular lobe and leveraging the pre-convoluted background for accurate decomposition, the proposed method represents a significant step towards integrating physically based rendering into the NeRF representation. The experiments demonstrate the superior performance of novel-view rendering compared to previous works, and the capability to re-render objects under arbitrary NeRF-style environments opens up exciting possibilities for bridging the gap between virtual and real-world scenes. The project and supplementary materials are available at https://yiyuzhuang.github.io/NeAI/.

==> supple.tex <==
% Start a new serial number
\setcounter{section}{0}

% Define a new number ordinal format
\renewcommand\thesection{\Alph{section}}
\renewcommand\thesubsection{\Alph{section}.\arabic{subsection}}

\section*{\Large \centering Supplementary Material}   % No serial number 

\section{Overview}
The supplementary material provides the derivation of integral lobe encoding (ILE, Eq. (6) in the submission) (Section \ref{sec:derivation}), the detailed architecture of our method, and the implementation details of the baseline methods (Section \ref{sec:implement}). We also introduce more details of our plug-and-play rendering process. The additional experiments demonstrate the superior performance of our method compared to the baseline methods (Section \ref{sec:experiment}). We \textbf{strongly} encourage the reader to see our website-video supplementary \gitlink, in which we present our results on various applications, especially our plug and play: place meshes in the public 360v2 datasets\footnote{\href{https://jonbarron.info/mipnerf360/}{https://jonbarron.info/mipnerf360/}} \cite{barron2022mip}. 

\section{Derivation of Integral Lobe Encoding}
\label{sec:derivation}

% The success of NeRF in high-fidelity rendering results is attributed to the proposed position encoding for learning high-frequency information. Each sample point $\mathbf{x}$ goes through this featurization procedure before fed into the MLP which is formulated as, 
% % $\left[  \sin(\mathbf{x}),\cos(\mathbf{x}),\ldots,\sin(2^{L-1}\mathbf{x}), \cos(2^{L-1}\mathbf{x})\right]^T$
%  \begin{equation}\small
%     \left[  \sin(\mathbf{x}),\cos(\mathbf{x}),\ldots,\sin(2^{L-1}\mathbf{x}), \cos(2^{L-1}\mathbf{x})\right]^T,
%  \end{equation}
% where $L$ is a hyperparameter and determines the bandwidth of the interpolation kernel. 
% This encoding enables the MLP parameterizing the scene to behave as an interpolation function, and maps the position into a high-frequency space.

Here, we introduce our ILE featurization procedure, in which we cast a lobe whose size is defined by the spatially-varying roughness. We feature conical frustums along that roughness-varying lobe. Similar to Mip-NeRF \cite{barron2021mip}, images in our method are rendered one pixel at a time so that we can describe our procedure in terms of an individual pixel of interest being rendered. Mip-NeRF casts a constant cone from the camera's center along the view direction that passes through the pixel's center, where the cone's size is spatially-constant and defined by the width of the pixel in world coordinates. As shown in Eq. (2) of the submission, we instead decompose the pixel's color into diffuse color and specular color of surface point $\mathbf{x}_s$, where $\mathbf{x}_s$ is the intersection between the object surface and the ray from the camera's center along the view direction. As shown in Eq. (5) of the submission, the specular color is the integration of the radiance field of each sampled point within the specular lobe combined with surface material. The apex of that specular lobe lies at $\mathbf{x}_s$, and the radius of the specular lobe is defined by $\hat{\rho}\hat{r}$. According to the pre-filtered environment map used in traditional CG rendering \cite{akenine2019real}, we set $\hat{\rho}$ to the material roughness $[0, 1]$ scaled by the pixel's size $r_0$, and set $\hat{r}$ to the width of the pixel $r_0$ scaled by mipmap levels (\ie resolution multi-scaling). In the implementation, we discretely divide the specular lobe into several conical frustums according to the discrete distance.
The set of positions $\mathbf{x}$ that lie within a conical frustum between two distant value $[t_0, t_1]$ is then defined as,
\begin{equation}\small
 \begin{split}
    F(\mathbf{x}, \mathbf{x}_s,\mathbf{l}_r,\rho,\hat{r},t_0,t_1)=\mathfrak{l}\left\{\left(t_0<\frac{\mathbf{l}_r^\top(\mathbf{x}-\mathbf{x}_s)}{\left\|\mathbf{l}_r\right\|^2_2}<t_1\right)\right.\\
    \wedge\left.\left(\frac{\mathbf{l}_r^\top(\mathbf{x}-\mathbf{x}_s)}{\left\|\mathbf{l}_r\right\|_2\left\|\mathbf{x}-\mathbf{x}_s\right\|_2}>\frac{1}{\sqrt{1+\left(\hat{\rho}\hat{r}/\|\mathbf{l}_r\|_2\right)^2}}\right)\right\},
\end{split}
\label{eq:concial_frustum}
\end{equation}
where $\mathfrak{l}\left\{\cdot\right\}$ is an indicator function: $F(\mathbf{x}, \cdot) = 1$ iff $\mathbf{x}$ is within the conical frustum defined by $(\mathbf{x}_s,\mathbf{l}_r,\rho,\hat{r},t_0,t_1)$. $\|\cdot\|_2$ refers to the Euclidean norm of a vector. Note that the conical frustum's radius is defined not only by the pixel width but also by the roughness, which means the roughness-varying specular lobe instead of constant.

Besides, the success of NeRF in high-fidelity rendering results is attributed to the proposed position encoding for learning high-frequency information. Each sample point $\mathbf{x}$ goes through this featurization procedure before being fed into the MLP, which is formulated as, 
% $\left[  \sin(\mathbf{x}),\cos(\mathbf{x}),\ldots,\sin(2^{L-1}\mathbf{x}), \cos(2^{L-1}\mathbf{x})\right]^T$
 \begin{equation}\small
    \mathrm{PE}(\mathbf{x}) \!=\! \left[  \sin(\mathbf{x}),\cos(\mathbf{x}),\ldots,\sin(2^{L-1}\mathbf{x}), \cos(2^{L-1}\mathbf{x})\right]^T,
    \label{eq:pe}
 \end{equation}
where $L$ is a hyperparameter and determines the bandwidth of the interpolation kernel. This encoding enables the MLP parameterizing the scene to behave as an interpolation function, and maps the position into a high-frequency space. Consequently, we establish a featurized representation of Eq. \eqref{eq:pe} inside the conical frustum defined by Eq. \eqref{eq:concial_frustum},
\begin{equation}\small
 \begin{split}
  \mathrm{ILE}(\mathbf{x}_s,\mathbf{l}_r, p_l)
  = \frac{\int A(\mathbf{x}, \mathbf{x}_s,\mathbf{l}_r) \mathrm{PE}(\mathbf{x}) {F}(\mathbf{x}, \mathbf{x}_s,\mathbf{l}_r,p_l)\mathrm{d}\mathbf{x}}
  {\int {F}(\mathbf{x}, \mathbf{x}_s,\mathbf{l}_r,p_l)\mathrm{d}\mathbf{x}},\\
  \mathrm{where}\ A(\mathbf{x}, \mathbf{x}_s,\mathbf{l}_r) = \exp{\left(\frac{\mathbf{l}_r^\top(\mathbf{x}-\mathbf{x}_s)}{\left\|\mathbf{l}_r\right\|_2\left\|\mathbf{x}-\mathbf{x}_s\right\|_2}-1\right)}
    \end{split}
    \label{eq:ILE_Int}
\end{equation}
where $p_l = \{\hat{\rho},\hat{r},t_0,t_1\}$ indicates the shape parameters about the conical frustum. According to Eq. (5) in the submission, a larger roughness corresponds to a rougher surface under a wider vMF distribution, and the integral volume is attenuated with the angle between incoming direction $\mathbf{l}={\mathbf{x}-\mathbf{x}_s}$ and the reflection direction $\mathbf{l}_r$ of the ambient illumination. Consequently, we consider the ILE must be under a vMF distribution, and it attenuates with the weights of $\mathbf{l}_r^\top(\mathbf{x}-\mathbf{x}_s)$. We then set the $A(\mathbf{x}, \mathbf{x}_s,\mathbf{l}_r)$ to the attenuation function, which can be well-approximated using a simple exponential function. Considering attenuation function $A$ is related to the direction of incoming illumination under a vMF distribution, the integral in the numerator can be defined via a multivariate Gaussian to efficiently represent the vMF attenuation and compute that features one time. 
According to integral position encoding (IPE) in Mip-NeRF \cite{barron2021mip}, the integration within a conical frustum in the numerator has no closed-form solution, only Gaussian approximation. However, this approximation will be inaccurate if there is a significant difference between the center and the boundary of the frustum. Compared to IPE, our ILE is the vMF attenuation, which is more suitable and accurate to describe as a multivariate Gaussian expression.

Eq. \eqref{eq:ILE_Int} can be directly simplified as a multivariate Gaussian. We first represent the shape of the conical frustum by the mean distance along the ray $\mu_t$, the variance along the ray $\sigma_t^2$, and the variance perpendicular to the ray $\sigma_r^2$. According to a midpoint $t_\mu=(t_0+t_1)/2$ and a half-width $t_\sigma=(t_1-t_0)/2$, these variables can be parameterized as,
 \begin{equation}\small
 \begin{split}
  \mu_t=t_\mu+\frac{2 t_\mu t_\delta^2}{3 t_\mu^2 + t_\delta^2},
  \sigma_t^2 = \frac{t_\sigma^2}{3} - \frac{4t_\delta^4(12t_\mu^2 - t_\sigma^2)}{15 (3 t_\mu^2+t_\delta^2)^2},
  \\
  \sigma^2_r(\hat{\rho}) = \hat{\rho}^2\hat{r}^2\left(\frac{t_\mu^2}{4}+ \frac{5t_\sigma^2}{12} - \frac{4t_\sigma^4}{15(3t_\mu^2+t_\delta^2)} \right),
  \end{split}
  \label{eq:cf_gaussian}
 \end{equation}
where the width of conical frustum $\sigma_r^2(\rho)$ is spatially varied with the roughness of surface point. 

We then compute the shape of a set of conical frustums along the specular lobe. We transform Eq. \eqref{eq:cf_gaussian} from the coordinate frame of conical frustums into the world coordinates, of which the mid-point $\mathbf{\mu}$ and variance $\mathbf{\Sigma}$ are defined as follows, 
\begin{equation}\small
    \mathbf{\mu}=\mathbf{x}_s+\mu_t\mathbf{l}_r,
    \mathbf{\Sigma}(\hat{\rho})=\sigma_t^2\left(\mathbf{l}_r\mathbf{l}_r^\top\right)+\sigma^2_r(\hat{\rho})\left(\mathbf{I}-\frac{\mathbf{l}_r\mathbf{l}_r^\top}{\left\|\mathbf{l}_r\right\|_2^2}\right),
    \label{eq:specular_lobe}
\end{equation}
where the variance $\mathbf{\Sigma}$ is related to spatially-varying roughness $\rho$. The next derivation is similar to Mip-NeRF \cite{barron2021mip}, Eq. \eqref{eq:pe} can be rewritten as matrix form ,
\begin{align}\small
    &\mathrm{PE}(\mathbf{x})=\left[\sin{(\mathbf{P}\mathbf{x}), \cos{(\mathbf{P}\mathbf{x})}}\right]^\top\\
    &\mathbf{P}\!\!=\!\!\left[
    \begin{matrix}
    1 & 0 & 0 & 2 & 0 & 0 & &2^{L-1} & 0 & 0\\
    0 & 1 & 0 & 0 & 2 & 0 & \cdots & 0 &2^{L-1} & 0 \\
    0 & 0 & 1 & 0 & 0 & 2 & & 0 & 0 &2^{L-1} \\
    \end{matrix}\right]^\top
    \label{eq:pe_mat}
\end{align}
This matrix form could help us to derive the final ILE feature. According to Eq. \eqref{eq:pe_mat}, we could identify the mean and covariance of the conical frustum Gaussian along the specular lobe. Our ILE feature can be finally formulated as the expected sines and cosines of the mean and the diagonal of the covariance matrix:
 \begin{equation}\small
 \begin{aligned}
\mathrm{ILE} ( \mathbf{x}_s,\mathbf{l}_r, p_l ) &= E_ {x\sim N(\mu,\mathbf{\Sigma}(\hat{\rho}))}[\mathrm{PE} (x)]
\\&= \left[ \begin{aligned}{\sin ( \mathbf{P}\mathbf{\mu} )\odot exp(-\frac{1}{2}\mathrm{diag}( \mathbf{P}\mathbf{\Sigma}(\hat{\rho})\mathbf{P}^T))}
\\{\cos ( \mathbf{P}\mathbf{\mu} )\odot exp(-\frac{1}{2}\mathrm{diag}( \mathbf{P}\mathbf{\Sigma}(\hat{\rho})\mathbf{P}^T))}   \end{aligned}\right],
 \end{aligned}
 \label{eq:ILE}
 \end{equation}
where $\odot$ refers to element-wise multiplication. For better understanding, we formulate Eq. \eqref{eq:ILE} as 
\begin{equation}\small
%        \mathrm{ILE} (\mathbf{x}_s, \mathbf{l}_r, \rho ) \!=\!\! 
        \mathrm{ILE}(\mathbf{x}_s,\mathbf{l}_r, p_l) \!=\! \left\lbrace \!
        \begin{bmatrix}
            {\sin( 2^{\ell}\mathbf{\mu} )\exp(-2^{\ell-1}\mathrm{diag}(\mathbf{\Sigma}(\hat{\rho})))} \\
            {\cos ( 2^{\ell}\mathbf{\mu})\exp(-2^{\ell-1}\mathrm{diag}(\mathbf{\Sigma}(\hat{\rho})))}   
        \end{bmatrix}\!
        \right\rbrace_{\ell=0}^{L-1},
    \label{eq:ILE_final}
\end{equation}
\begin{equation}\small
    \mathrm{diag}(\mathbf{\Sigma}(\hat{\rho}))=\sigma_t^2\left(\mathbf{l}_r\odot\mathbf{l}_r\right)+\sigma^2_r(\hat{\rho})\left(\mathbf{1}-\frac{\mathbf{l}_r\odot\mathbf{l}_r}{\left\|\mathbf{l}_r\right\|_2^2}\right)
\end{equation}
where $L$ is a hyperparameter and determines the bandwidth of the interpolation kernel. $p_l = \{\hat{\rho},\hat{r},t_0,t_1\}$ refers to the shape parameters about the conical frustum.  Our ILE allows the MLP to parameterize the incoming illumination inside the roughness-varying specular lobe, whose strength is variable with the incoming direction under vMF distribution, to behave as an interpolation function. As a result, our ILE efficiently maps continuous input coordinates into a high-frequency space.


\begin{figure}[h]
\centering
% \includegraphics[width=\linewidth]{}
\includegraphics[width=0.7\linewidth]{Figure/fig_network.pdf}
\caption{Details of the network architecture. As for the material network, a ReLU is applied for each MLP except the last layer. We choose tanh and sigmoid to the output of $\mathbf{C}_d$ and ${\alpha, \rho}$, separately. The  parameters of illumination network is the same as \cite{barron2021mip}. }
\label{fig:network}
\end{figure}
\section{Implement Details}
\label{sec:implement}

\begin{figure}[th]
\centering
\includegraphics[width=\linewidth]{Figure/for_cmp_all.pdf}
\caption{Visualisations of the results on our "Glossy Blender" dataset. It' is obvious that the reflection and the highlights are correctly reconstructed with our method. Compared to NeILF or other baselines, it shows great robustness in representing complex lighting.
 } 
% \label{fig:dataset}
\label{fig:cmp_blender}
\end{figure}

\begin{figure*}[th]
\centering
\includegraphics[width=\linewidth]{Figure/comp_blendedMVS_row_2.pdf}
\caption{More qualitative comparison with zoom-in details of our method against baselines on real-world \cite{yao2020blendedmvs, park2020seeing} dataset. Our method produces the most visually pleasing novel views, especially on reconstructing the highlight regions and detailed textures, as shown in zoom-in details. Note that the decomposed diffuse results of our method are also presented, where the highlights are successfully removed.  The diffuse color of our method looks wrong on white balance, probably because lacking of enough background information.
 }
% \label{fig:dataset}
\label{fig:cmp_real}
\end{figure*}



\subsection{Architecture}
In the paper, we introduce our novel representation of illumination, and the rendering equation for the pixel of the object is given as Eq. (7). The whole pipeline is differentiable, and the architecture of the network is shown in Fig. \ref{fig:network}. We believe the architecture can be easily re-implemented or extended by other researchers.

For the pixel of the background, we remove the diffuse term $\mathbf{C}_d$ and the tint $\alpha$, and directly give the value of radius $r_p=3\sigma r_0$. $\sigma$ is set according to the pre-convoluted image. It is worth noting that, different with traditional pre-filtered technique \cite{akenine2019real}, our method does not handle the images with different mipmap levels (multiscale resolution) for simplification, as shown in Fig. 3, so $\hat{r}$ is set to the raw pixel's size $r_0$.
According to Eq. (3) and ILE Eq. \eqref{eq:ILE_final}, the captured value of along the ray $\mathbf{r}(t)=\mathbf{o}+ t \mathbf{d}$ from $t_n$ to $t_f$ is:
\begin{equation}\small
\begin{aligned} \label{eq:rendering}
 \mathbf{C}(\mathbf{o},\mathbf{d}) &= \int_{t_n}^{t_f}{T(t)\sigma(\mathcal{L}})  \mathbf{C}(\mathcal{L},\mathbf{d})\mathrm{d}t ,
\\
 	\textup{where} \:
 	\mathcal{L} &= \mathrm{ILE}(\mathbf{r}(t),\mathbf{d},p_l),
\end{aligned}
\end{equation}
and $p_l = \{3\sigma,r_0,t_n,t_f\}$ refers to the shape parameters about the conical frustum along that ray.




\subsection{More about Plug and Play} With our novel representation of environment lighting and its interaction with the object surface, we lay the foundation for a fancy application: seamless illumination of a decomposed mesh with a NeRF-style environment.
 % Since we have well decoupled lighting and materials, this lays the groundwork for a fancy application, that is moving our plug-and-play models of objects into another NeRF-like environment. 
 For a decomposed object from stage two, we need to manually set the transformation to put it into the environment.
% Transformation to move our objects into the environment needs to be set manually.
Sequentially, the realistic results can be rendered through the rendering equations shown in Eq. (7) of the submission and Eq. \eqref{eq:rendering}. 
Considering that the object is sometimes occluded by the landscape, we modify the rendering Eq.(7) slightly to account for occlusions during the rendering of new views,
\begin{equation}\small
    \mathbf{C}(\mathbf{o}, \mathbf{d}) \!=\!  
        \mathbf{C^*}(\mathbf{o},\mathbf{d})  w^*(\mathbf{o},\mathbf{d}) 
        + \mathbf{C}( \mathbf{x}_s,  \mathbf{d}) (1-w^*(\mathbf{o},\mathbf{d})),
\end{equation}
where $\mathbf{C^*(\cdot)}$ and $w^*(\cdot)$ with superscript * mean that the $t_f$ is set to $0.99$ times the depth of the object's surface. $w^*(\cdot)$ is the cumulative distribution function of density from $t_n$ to $t_f$ along the ray. Additionally, it is recommended to scale the decomposed material $\alpha,\rho,\mathbf{C}_d$ for better visual effect. The rendering videos could be found in \textit{supplement website}.

It is worth noting that, with our rendering pipeline, our method takes about 50 seconds to render an $800\times800$ image on a single Tesla A100, while the Cycles engine on Blender \cite{blender} takes about several minutes to render the ground truth.

\subsection{Traning Details}
Our implementation is based on the re-implementation pytorch \cite{Pytorch} of Mip-NeRF \cite{barron2021mip}.
We train our model with Adam \cite{kingma2015adam} for 1 million iterations.
For each iteration, 4096 rays are randomly selected from all images including the pre-convoluted images. The training process takes about two days to train on a single Tesla A100 GPU or 16 hours for 600,000 iterations on 4 Tesla A100 GPUs.




\subsection{Baseline Implementations}
\noindent\textbf{NeILF. \cite{yao2022neilf}} We follow the same setup in the author's code\footnote{\href{https://github.com/apple/ml-neilf}{https://github.com/apple/ml-neilf}}. The architecture can be divided into two parts, one for material estimation, called BRDF MLP, and the other, NEILF MLP. We follow their procedure for training on a single scene.

\noindent\textbf{NeILF$^*$.} We replace the BRDF MLP with our material network and modify the rendering equation to directly predict the diffuse term as $\mathbf{C}_d$. Another change is to modify the Fresnel term F to be a position-dependent magnitude $\alpha$, so the specular term is only related to roughness $\rho$, magnitude $\alpha$. The predicted $\mathbf{C}_s$ is finally obtained by integrating with the product of all incident light and the specular term on the hemisphere $\Omega$.
% $f_s(=(D(\mathbf{h};r)F(\mathbf{w}_o,\mathbf{h};\mathbf{b},m)\cdot G(\mathbf{w}_i,\mathbf{w}_o,\mathbf{h};r)$

\noindent\textbf{Ne-Env.} A variant of NeILF$^*$, named neural environment map. The position point input of NEILF MLP is removed, so the spatially-varying environment map is modified to the non-spatially varying environment map.

% \zyy{is it reasonable to introduce our ablation experiment setup here?}
\noindent\textbf{w/o ILE.} The roughness $\rho$ is set to a small constant as $r_0$, which means the adaptive lobe encoding is abolished, and the specular lobe degenerates into a thin ray. It causes artifacts to the objects with rough material. 

\section{Additional Results}
\label{sec:experiment}
\subsection{Glossy Blender dataset}



The error metrics for each individual scene are provided in Tabs. \ref{tab:quan_glossy_psnr}, \ref{tab:quan_glossy_ssmi} and \ref{tab:quan_glossy_lpips}, and the more visualized results are shown in Fig. \ref{fig:cmp_blender}. It demonstrates the significantly superior performance of our lighting representation compared to the baselines through rendering quality on novel views.  

We also show visual comparison of the ablation in Fig. \ref{fig:ablation}. We can see that, without the Bilateral Smoothness regularization (Eq. (8) in our submission), although obtains the best metric performance, it generates noise and becomes inconsistent across the same material. It is unsuitable for material editing applications. On the other hand, without the ILE, spatially-varying roughness can not be handled very well, resulting in artifacts of diffuse items, as shown in Fig. \ref{fig:ablation}. The result of 'w/o BG' shows that without the assistance of the background, it's easy to creates ambiguity between light and material.

% The visualization of pre-convoluted input images can be found in Fig. \ref{fig:pre-convoluted}.


\begin{figure}[th]
\centering
% \includegraphics[width=\linewidth]{}
\includegraphics[width=\linewidth]{Figure/Fig_ablation.pdf}
\caption{Visualizations of the decomposed material for ablation study. Without the Bilateral Smoothness regularization, the material becomes noisy. Without the ILE, changes in material roughness cannot be handled well, resulting in artifacts of diffuse items. Without background, the roughness is not correct due to the effects of lighting.
 }

\label{fig:ablation}
\end{figure}


\subsection{Real-world dataset}




Tabs. \ref{tab:quan_synth_ssim} and \ref{tab:quan_synth_lpips} list the average SSIM and LPIPS for each individual scene in real-world dataset \cite{yao2020blendedmvs, park2020seeing}, and more visulization is shown in Fig. \ref{fig:cmp_real}. It demonstrates the performance of our method in real scenes compared to NeILF and its variants in terms of rendering quality on novel views. 
% We abbreviate a few words to cut the length of the table, T-tearoom, P-playroom, B-bedroom. 

% \subsection{Qualitative comparison for Ablation}
% We show the qualitative comparison in Fig. \ref{fig:ablation}.




\begin{table}[tb] 
\centering
\caption{Per-Scene quantitative comparison of SSIMs on real-world dataset.}
% \small
\scriptsize 
\begin{tabularx}{\linewidth}{@{}l|CCCCCCCC}
\hline
                   &bull      &cam       &stone       &gold         &conch          & vase                          &cans    &chips\\ \hline
 NeILF             &\cc{1}0.779     &0.460     &\cc{2}0.859      &\cc{1}0.771       &\cc{1}0.787  &\cc{2}0.827      &\cc{2}0.957  &\cc{2}0.939             \\
 NeILF$^*$         &0.725         &\cc{2}0.573     &0.801        &0.625          &0.744           &0.745             &0.949  &0.917   \\
Ne-Env             &0.745         &0.567     &0.801              &0.633           &0.750         &0.738             &0.944  &0.915  \\
%  Ours                            & 37.931 & 0.981  & xxx           \\
 Ours               &\cc{2}0.760   &\cc{1}0.705   & \cc{1}0.862   &\cc{2}0.769     &\cc{2}0.655     &\cc{1}0.851     &\cc{1}0.960  &\cc{1}0.953      \\\hline
\end{tabularx}
\label{tab:quan_synth_ssim}
\end{table}



\begin{table}[thb] 
\centering
\caption{Per-Scene quantitative comparison of LPIPS on real-world dataset.}
% \small
\scriptsize 
\begin{tabularx}{\linewidth}{@{}l|CCCCCCCC}
\hline
                   &bull      &cam       &stone       &gold      &conch     & vase                                   &cans    &chips\\ \hline
 NeILF             &\cc{2}0.272     &0.437    &\cc{2}0.131      &\cc{1}0.173      &\cc{1}0.313     &\cc{2}0.213      &\cc{2}0.034  &\cc{2}0.051            \\
 NeILF$^*$         &0.318        &\cc{2}0.345  &0.172           &0.297             &0.382     &0.301                 &0.044  &0.076 \\
Ne-Env             &0.324        &0.355        &0.187           &0.311              &0.391     &0.311                 &0.050  &0.082 \\
%  Ours                            & 37.931 & 0.981  & xxx           \\
 Ours               &\cc{1}0.257   &\cc{1}0.256   &\cc{1}0.130      &\cc{2}0.186        &\cc{2}0.366     &\cc{1}0.172    &\cc{1}0.028  &\cc{1}0.041       \\\hline
\end{tabularx}
\label{tab:quan_synth_lpips}
\end{table}



\begin{figure}[th]
\centering
\includegraphics[width=1\linewidth]{Figure/Fig_diss_geo.pdf}
\caption{Qualitative and quantitative results based on a geometry reconstructed by IDR\cite{yariv2020multiview} (in column 2,3). Compared to the result of the ideal test (in column 4), it is worth noting that the geometric deviation from the stage one would affects the quality of novel-view synthesis. This is because the tracing direction and origin of the specular lobe depends on the geometry. For a rougher surface, the lobe is wider, so is has more tolerance to this perturbation. The opposite is true for a smoother surface. We demonstrate this effect with two examples of different roughness.
 }

% \label{fig:dataset}
\label{fig:geometry_disc}
\end{figure}


\begin{table*}[t]%[ht] 
\centering
\caption{Per-Scene quantitative comparison of PSNRs on Glossy Blender dataset.}
% \scriptsize 
\small
\begin{tabularx}{\linewidth}{@{}l|CCCCCCC}
\hline
                   & Car  &Helmet & Coffee  &RedBall    & GoldBall & GoldBall & MetalBall  \\ 
                   & Playroom  &Bedroom & Tearoom  &Playroom    & Bedroom & Bedroom2 & Tearoom  \\
\hline
 NeILF             & 20.863   & 28.282    &26.785      &26.630         &24.889         &24.620        &28.886        \\
 NeILF$^*$         & 21.332   & 29.419    &27.036      &27.444         &25.383         &25.175        &29.216  \\
Ne-Env             & 21.326   & 29.228    & 26.953     &26.777          &24.682         &24.542       &28.287     \\
%  Ours                            & 37.931 & 0.981  & xxx           \\
\hline
w/o ILE             &35.090    &38.843     & 41.407     &38.046        &35.489        &34.544        &38.116            \\
w/o background             &35.131    &39.835     & 40.496     &37.649        &35.562        &34.893         &31.263            \\
w/o pre-convolution             & 35.072   & 39.608   & 41.559      &38.567        &35.987        &35.110         &38.336          \\
%  w/o bilateral smoothness        & 38.166   & 0.983  & 0.029      \\
 w/o  regularization          & \cc{1}35.983    & \cc{1}41.439   & \cc{1}42.167    &\cc{1}39.004          &\cc{1}36.429       &\cc{1}35.535         &\cc{1}38.540
 \\  
 Ours               & \cc{2}35.296    & \cc{2}39.868   & \cc{2}41.735        &\cc{2}38.840         &\cc{2}36.301         &\cc{2}35.346         &\cc{2}38.506         \\\hline
\end{tabularx}
% \vspace{-0.6}
\label{tab:quan_glossy_psnr}
\end{table*}

\begin{table*}[h]%[hb] 
\centering
\caption{Per-Scene quantitative comparison of SSMIs on Glossy Blender dataset.}
\small
\begin{tabularx}{\linewidth}{@{}l|CCCCCCC}
\hline
                   & Car  &Helmet & Coffee  &RedBall    & GoldBall & GoldBall & MetalBall  \\
                   & Playroom  &Bedroom & Tearoom  &Playroom    & Bedroom & Bedroom2 & Tearoom  \\
\hline
 NeILF             & 0.908    & 0.942     &0.966      &0.917         &0.917          &0.913         &0.947         \\
 NeILF$^*$         & 0.926    & 0.955     &0.969       &0.924          &0.924 
         &0.922         &0.950   \\
Ne-Env             &0.926    & 0.954     & 0.969     &0.918         &0.917          &0.915      &0.946      \\
%  Ours                            & 37.931 & 0.981  & xxx           \\
\hline
w/o ILE        &\cc{2}0.970     &0.981       &\cc{2}0.982      &0.982       &0.981         &0.978          &0.981 \\  
w/o background              &\cc{2}0.970     &0.988      & 0.981      &0.980       &0.982         &\cc{2}0.981          &0.971            \\
w/o pre-convolution             &0.969    &\cc{2}0.985    &\cc{2}0.982       &0.985         &0.982         &0.980         &\cc{1}0.982           \\
%  w/o bilateral smoothness        & 38.166   & 0.983  & 0.029      \\
 w/o  regularization          & \cc{1}0.973     & \cc{1}0.990    & \cc{1}0.983    &\cc{1}0.986          &\cc{1}0.984      &\cc{1}0.982          &\cc{1}0.982 
 \\  
 Ours               &0.968     & \cc{2}0.985   &0.981    &\cc{1}0.986         &\cc{2}0.983          &\cc{2}0.981         &\cc{1}0.982         \\\hline
\end{tabularx}
% \vspace{-0.6}
\label{tab:quan_glossy_ssmi}
\end{table*}


\begin{table*}[!htbp]%[h] 
\centering
\caption{Per-Scene quantitative comparison of LPIPS on Glossy Blender dataset.}
\small
\begin{tabularx}{\linewidth}{@{}l|CCCCCCC}
\hline
                   & Car  &Helmet & Coffee  &RedBall    & GoldBall & GoldBall & MetalBall  \\
                   & Playroom  &Bedroom & Tearoom  &Playroom    & Bedroom & Bedroom2 & Tearoom  \\
\hline
 NeILF             & 0.115    &0.081     &0.056       &0.096          &0.099          &0.108         &0.057         \\
 NeILF$^*$         &0.109    &0.073     &0.062       &0.094          &0.095          &0.098         &0.060  \\
Ne-Env             &0.110    &0.074     &0.063     &0.095           &0.098         &0.102        &0.062      \\
%  Ours                            & 37.931 & 0.981  & xxx           \\
\hline
w/o ILE             &0.049      &0.047      &\cc{1}0.045      &0.025       &0.025        &0.027          &\cc{1}0.030            \\
w/o background              & \cc{2}0.048     &\cc{2}0.027      &0.048      &0.026       &\cc{1}0.019        &\cc{2}0.021          &0.038            \\
w/o pre-convolution             &0.054    & 0.034    & 0.046       &0.019            &0.021         &0.023         &\cc{1}0.030           \\
%  w/o bilateral smoothness        & 38.166   & 0.983  & 0.029      \\
 w/o  regularization          & \cc{1}0.047     & \cc{1}0.025   & \cc{1}0.045     &\cc{1}0.017          &\cc{1}0.019        &\cc{1}0.020          &\cc{1}0.030 
 \\  
 Ours               &0.057           &0.036        & 0.046      &\cc{2}0.018          &0.021          &\cc{2}0.021          &\cc{1}0.030          \\\hline
\end{tabularx}
% \vspace{-0.6}
\label{tab:quan_glossy_lpips}
\end{table*}


\subsection{Discussion about the geometric perturbation.}


Previous studies have shown that the decomposition between light and material relies on the geometric quality \cite{park2020seeing, yao2022neilf, zhang2022modeling}.
In Section 4 of the main text, we adopt the rendered depth and normal maps as the result of stage one to isolate the influence of geometry quality. This means that the quality of novel-view synthesis will only reflect the lighting reconstruction and material decomposition.
However, in practice, there is always some deviation in geometry. Few studies have discussed the impact and underlying reason for this dependency. Through the experiment, we find that the decomposition of the mirror-like surfaces is more sensitive to the geometric perturbation, as shown in Fig. \ref{fig:geometry_disc}. This because our physically based lobe tracing relies on the reconstructed geometry to calculate the incoming direction. If the estimated geometry deviates from the true geometry, different tracing lobes may conflict with each other, which becomes more serious when the lobe is thinner. 
Despite this challenge, our method still produces better results of novel-view synthesis than existing methods, which demonstrates its robustness to geometric perturbation. 
Moreover, we suggest that this error could be potentially exploited to reconstruct a more accurate geometry in the future work.


\begin{figure*}[thb]
\centering
% \includegraphics[width=\linewidth]{}
\includegraphics[width=0.8\linewidth]{Figure/Fig_dataset.png}
\caption{Visualizations of the our new “Glossy Blender" scenes. Each one is rendered by a camera under the ceiling with a focal length of around 12mm.
 }
\label{fig:dataset}
\end{figure*}

\subsection{Dataset License}
We overview each scene in Fig. \ref{fig:dataset}. Our new ``Glossy Blender'' scenes were adapted from the following Sketchfab \href{https://sketchfab.com/feed}{https://sketchfab.com/feed} models, including object models and ambient illumination models. \\The object models are:
\begin{enumerate}
    \item Car: created by \emph{DAVID.3D.ART}, CC Attribution-NonCommercial license (model \emph{AC-Bmw 1m});
    \item Helmet: released by public NeILF dataset \cite{yao2022neilf};
    \item Coffee: created by \emph{Elen}, CC Attribution-ShareAlike license (model \emph{Coffee cup with plate});
    \item GoldBall \& RedBall \& MetaBall: released by public NeRF blender dataset \cite{mildenhall2020nerf} (model \emph{materials dataset}).
\end{enumerate}
The ambient illumination models are:
\begin{enumerate}
    \item Tearoom: created by \emph{Anex}, CC Attribution license (model \emph{Room});
    \item Playroom: created by \emph{enteRenders}, CC Attribution license (model \emph{Interior Living Room Corner});
    \item Bedroom \& Bedroom2: created by \emph{ankitk2618}, CC Attribution license (model \emph{Bedroom Interior}).
    % \item BedRoom2: created by \emph{ankitk2618}, CC Attribution license (model \emph{Bedroom Interior});
\end{enumerate}
We have slightly remixed, transformed, and built upon the material of models for better visual harmonization between objects and ambient illuminations. 


\noindent\textbf{Acknowledgements. }
This work was supported by the NSFC grant 62001213, 62025108, and a gift funding from Tencent Rhino-Bird Research Program.

